Design, Kinematics, and Deployment of a Continuum Underwater Vehicle-Manipulator System

Underwater vehicle-manipulator systems (UVMSs) are underwater robots equipped with one or more manipulators to perform intervention missions. This paper provides the mechanical, electrical, and software design of a novel UVMS equipped with a continuum manipulator, referred to as a continuum-UVMS. A kinematic model for the continuum-UVMS is derived in order to build an algorithm to resolve the robot's redundancy and generate joint space commands. Different methods to optimize the trajectory for specific tasks are proposed using both the weighted least norm solution and the gradient projection method. Kinematic simulation results are analyzed to assess the performance of the proposed algorithm. Finally, the continuum-UVMS is deployed in an experimental demonstration in which both teleoperation and autonomous control are tested for a given reference trajectory.

==> Makefile <==
PAPER := journal2024_underwater_redundancy

createfolder:
	mkdir -p pdf

paper:
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	bibtex pdf/$(PAPER).aux; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \

clean:
	rm -f pdf/*; \
	rm -f *.bbl; \
	rm -f $(PAPER)_arxiv.tgz; \

clean_temp_files:
	rm -f pdf/*.dvi
	rm -f pdf/*.ps
	rm -f pdf/*.aux
	rm -f pdf/*.fdb_latexmk
	rm -f pdf/*.fls
	rm -f pdf/*.log
	rm -f pdf/*.out
	rm -f pdf/*.bbl
	rm -f pdf/*.blg
	rm -f pdf/*.toc

arxiv: paper
	rm -f $(PAPER)_arxiv.tgz; \
	touch $(PAPER)_arxiv.tgz; \
	cp pdf/$(PAPER).bbl ./ms.bbl; \
	tar --exclude=$(PAPER)_arxiv.tgz -cvzf $(PAPER)_arxiv.tgz --exclude-vcs --exclude=extra --exclude=download --exclude=bib --exclude=pdf --exclude=Makefile --exclude=*~ .

all: \
	createfolder \
	paper \
	arxiv \
	clean_temp_files
